DORI: Distributed Outdoor Robotic Instruments

DORI (Distributed Outdoor Robotic Instruments) is a remotely controlled vehicle that is designed to simulate a planetary exploration mission. DORI is equipped with over 20 environmental sensors and can perform basic data analysis, logging and remote upload. The individual components are distributed across a fault-tolerant bus for redundancy. A partial sensor list includes atmospheric pressure, rainfall, wind speed, GPS, gyroscopic inertia, linear acceleration, magnetic field strength, temperature, laser and ultrasonic distance sensing, as well as digital audio and video capture. The project uses recycled consumer electronics devices as a low-cost source for sensor components. This report describes the hardware design of DORI including sensor electronics, embedded firmware, and physical construction.

==> files/ack.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `ack.tex' --- aknowledgments for thes-full.tex, thes-short-tex from
%%               the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Acknowledgment 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\prefacesection{Acknowledgments}
Here go all the people you want to thank.










==> files/appone.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `appone.tex' --- 1st appendix for thes-full.tex, thes-short-tex from
%%                  the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%        Appendix 1
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{Safety}\label{app:spacing}
\index{appendices}\index{sectioning}


==> files/apptwo.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `apptwo.tex' --- 2nd appendix for thes-full.tex from
%%                  the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%        Appendix 2
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{Acknowledgements}\label{app:lists}
\index{formatting of Lists}
petit fat elmchan

==> files/bibl.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `bibl.tex' --- bibliography for thes-full.tex, thes-short-tex from
%%                the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Bibliography
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nocite{*}     % everything cited automatically

\renewcommand{\baselinestretch}{\tighttextstretch} %% get smaller spacing
\normalsize

\bibliographystyle{plain}   %% dash under repeated name, von ignored
\addcontentsline{toc}{chapter}{Bibliography}
\typeout{Bibliography}
\bibliography{files/thes-both}
\renewcommand{\baselinestretch}{\textstretch} %% get normal spacing
\normalsize



==> files/dedquot.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `dedquot.tex' --- dedication and quotation for thes-full.tex from
%%                   the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Dedication/Quotation pages
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\dedication{To whomever whoever reads this!}
\thesquot{%
``Don't worry, Gromit. Everything's under control!''\\[5pt]%
--- The Wrong Trousers, \textsc{Aardman Animations}, 1993%
}

%%% generate pages
\dedicquotation


==> files/ind.tex <==
%% Copyright 1998 Pepe Kubon
%%
%% `ind.tex' --- index for thes-full.tex from
%%               the `csthesis' bundle
%%
%% You are allowed to distribute this file together with all files
%% mentioned in READ.ME.
%%
%% You are not allowed to modify its contents.
%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Index
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\baselinestretch}{\tighttextstretch} %% get smaller spacing
\normalsize

\addcontentsline{toc}{chapter}{Index}
\typeout{Index}
\printindex

\renewcommand{\baselinestretch}{\textstretch} %% get normal spacing
\normalsize



==> img/wind.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\multiput(294.00,233.92)(30.709,-0.493){23}{\rule{23.946pt}{0.119pt}}
\multiput(294.00,234.17)(725.299,-13.000){2}{\rule{11.973pt}{0.400pt}}
\multiput(1202.43,292.92)(-0.953,-0.499){141}{\rule{0.861pt}{0.120pt}}
\multiput(1204.21,293.17)(-135.213,-72.000){2}{\rule{0.431pt}{0.400pt}}
\put(294.0,235.0){\rule[-0.200pt]{0.400pt}{99.010pt}}
\put(254,372){\makebox(0,0)[r]{ 510}}
\put(294.0,372.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,412){\makebox(0,0)[r]{ 520}}
\put(294.0,412.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,451){\makebox(0,0)[r]{ 530}}
\put(294.0,451.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,489){\makebox(0,0)[r]{ 540}}
\put(294.0,489.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,528){\makebox(0,0)[r]{ 550}}
\put(294.0,528.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,568){\makebox(0,0)[r]{ 560}}
\put(294.0,568.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,607){\makebox(0,0)[r]{ 570}}
\put(294.0,607.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(254,646){\makebox(0,0)[r]{ 580}}
\put(294.0,646.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(1066,836){\makebox(0,0)[r]{Vertical}}
%\put(1066,756){\makebox(0,0)[r]{Vertical}}
\put(1136,836){\makebox(0,0){$+$}}
\put(417,404){\makebox(0,0){$+$}}
\put(417,404){\makebox(0,0){$+$}}
\put(443,424){\makebox(0,0){$+$}}
\put(443,424){\makebox(0,0){$+$}}
\put(443,404){\makebox(0,0){$+$}}
\put(521,413){\makebox(0,0){$+$}}
\put(521,413){\makebox(0,0){$+$}}
\put(475,403){\makebox(0,0){$+$}}
\put(501,423){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(456,413){\makebox(0,0){$+$}}
\put(423,394){\makebox(0,0){$+$}}
\put(385,405){\makebox(0,0){$+$}}
\put(417,424){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(385,444){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(495,453){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(443,424){\makebox(0,0){$+$}}
\put(443,404){\makebox(0,0){$+$}}
\put(417,404){\makebox(0,0){$+$}}
\put(443,404){\makebox(0,0){$+$}}
\put(443,424){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(514,463){\makebox(0,0){$+$}}
\put(514,463){\makebox(0,0){$+$}}
\put(514,444){\makebox(0,0){$+$}}
\put(482,444){\makebox(0,0){$+$}}
\put(482,464){\makebox(0,0){$+$}}
\put(495,453){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(456,464){\makebox(0,0){$+$}}
\put(437,454){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(482,464){\makebox(0,0){$+$}}
\put(514,463){\makebox(0,0){$+$}}
\put(514,463){\makebox(0,0){$+$}}
\put(482,464){\makebox(0,0){$+$}}
\put(482,444){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(482,444){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(501,442){\makebox(0,0){$+$}}
\put(501,442){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(417,444){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(437,454){\makebox(0,0){$+$}}
\put(424,445){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(521,433){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(443,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(437,434){\makebox(0,0){$+$}}
\put(456,425){\makebox(0,0){$+$}}
\put(514,424){\makebox(0,0){$+$}}
\put(514,424){\makebox(0,0){$+$}}
\put(456,425){\makebox(0,0){$+$}}
\put(482,424){\makebox(0,0){$+$}}
\put(514,424){\makebox(0,0){$+$}}
\put(482,444){\makebox(0,0){$+$}}
\put(482,464){\makebox(0,0){$+$}}
\put(463,453){\makebox(0,0){$+$}}
\put(475,443){\makebox(0,0){$+$}}
\put(1066,785){\makebox(0,0)[r]{Light wind}}
%\put(1066,715){\makebox(0,0)[r]{Light wind}}
\put(1136,785){\makebox(0,0){$\times$}}
\put(843,628){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(856,574){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(741,596){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(856,618){\makebox(0,0){$\times$}}
\put(817,629){\makebox(0,0){$\times$}}
\put(805,640){\makebox(0,0){$\times$}}
\put(843,628){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(804,608){\makebox(0,0){$\times$}}
\put(778,608){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(766,619){\makebox(0,0){$\times$}}
\put(785,629){\makebox(0,0){$\times$}}
\put(863,639){\makebox(0,0){$\times$}}
\put(843,628){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(843,585){\makebox(0,0){$\times$}}
\put(863,595){\makebox(0,0){$\times$}}
\put(817,586){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(766,619){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(856,618){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(785,586){\makebox(0,0){$\times$}}
\put(805,616){\makebox(0,0){$\times$}}
\put(817,605){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(843,605){\makebox(0,0){$\times$}}
\put(837,639){\makebox(0,0){$\times$}}
\put(817,605){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(778,565){\makebox(0,0){$\times$}}
\put(785,555){\makebox(0,0){$\times$}}
\put(759,555){\makebox(0,0){$\times$}}
\put(785,555){\makebox(0,0){$\times$}}
\put(837,584){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(856,618){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(766,619){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(741,596){\makebox(0,0){$\times$}}
\put(741,576){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(766,576){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(766,596){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(824,595){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(798,575){\makebox(0,0){$\times$}}
\put(843,585){\makebox(0,0){$\times$}}
\put(843,585){\makebox(0,0){$\times$}}
\put(817,586){\makebox(0,0){$\times$}}
\put(805,596){\makebox(0,0){$\times$}}
\put(817,586){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
\put(843,585){\makebox(0,0){$\times$}}
\put(843,605){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(824,618){\makebox(0,0){$\times$}}
\put(798,619){\makebox(0,0){$\times$}}
\put(766,619){\makebox(0,0){$\times$}}
\put(766,619){\makebox(0,0){$\times$}}
\put(798,595){\makebox(0,0){$\times$}}
\put(824,575){\makebox(0,0){$\times$}}
%\put(1066,674){\makebox(0,0)[r]{Strong wind}}
\put(1066,734){\makebox(0,0)[r]{Strong wind}}
\sbox{\plotpoint}{\rule[-0.400pt]{0.800pt}{0.800pt}}%
\put(1136,734){\makebox(0,0){$\ast$}}
\put(1070,655){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1057,685){\makebox(0,0){$\ast$}}
\put(1077,696){\makebox(0,0){$\ast$}}
\put(1051,696){\makebox(0,0){$\ast$}}
\put(999,686){\makebox(0,0){$\ast$}}
\put(1012,676){\makebox(0,0){$\ast$}}
\put(979,656){\makebox(0,0){$\ast$}}
\put(979,637){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(979,637){\makebox(0,0){$\ast$}}
\put(1012,656){\makebox(0,0){$\ast$}}
\put(1057,666){\makebox(0,0){$\ast$}}
\put(1077,676){\makebox(0,0){$\ast$}}
\put(1031,686){\makebox(0,0){$\ast$}}
\put(979,676){\makebox(0,0){$\ast$}}
\put(992,665){\makebox(0,0){$\ast$}}
\put(1018,665){\makebox(0,0){$\ast$}}
\put(992,665){\makebox(0,0){$\ast$}}
\put(960,646){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1037,636){\makebox(0,0){$\ast$}}
\put(1037,636){\makebox(0,0){$\ast$}}
\put(1037,656){\makebox(0,0){$\ast$}}
\put(1070,675){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(953,677){\makebox(0,0){$\ast$}}
\put(953,677){\makebox(0,0){$\ast$}}
\put(1012,676){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1037,656){\makebox(0,0){$\ast$}}
\put(1031,666){\makebox(0,0){$\ast$}}
\put(1031,666){\makebox(0,0){$\ast$}}
\put(1096,655){\makebox(0,0){$\ast$}}
\put(1122,674){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(979,676){\makebox(0,0){$\ast$}}
\put(1037,656){\makebox(0,0){$\ast$}}
\put(1096,635){\makebox(0,0){$\ast$}}
\put(1089,646){\makebox(0,0){$\ast$}}
\put(1051,676){\makebox(0,0){$\ast$}}
\put(1051,696){\makebox(0,0){$\ast$}}
\put(1051,696){\makebox(0,0){$\ast$}}
\put(1018,697){\makebox(0,0){$\ast$}}
\put(1077,696){\makebox(0,0){$\ast$}}
\put(1109,695){\makebox(0,0){$\ast$}}
\put(1077,676){\makebox(0,0){$\ast$}}
\put(999,647){\makebox(0,0){$\ast$}}
\put(953,657){\makebox(0,0){$\ast$}}
\put(999,686){\makebox(0,0){$\ast$}}
\put(1018,697){\makebox(0,0){$\ast$}}
\put(1051,676){\makebox(0,0){$\ast$}}
\put(1051,657){\makebox(0,0){$\ast$}}
\put(1031,647){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1037,636){\makebox(0,0){$\ast$}}
\put(1037,636){\makebox(0,0){$\ast$}}
\put(979,637){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(979,637){\makebox(0,0){$\ast$}}
\put(999,647){\makebox(0,0){$\ast$}}
\put(1057,646){\makebox(0,0){$\ast$}}
\put(1057,646){\makebox(0,0){$\ast$}}
\put(1031,647){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(999,647){\makebox(0,0){$\ast$}}
\put(993,658){\makebox(0,0){$\ast$}}
\put(1018,657){\makebox(0,0){$\ast$}}
\put(1018,657){\makebox(0,0){$\ast$}}
\put(1031,647){\makebox(0,0){$\ast$}}
\put(1037,656){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1037,656){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1012,636){\makebox(0,0){$\ast$}}
\put(1037,636){\makebox(0,0){$\ast$}}
\put(1018,645){\makebox(0,0){$\ast$}}
\put(1031,654){\makebox(0,0){$\ast$}}
\put(998,655){\makebox(0,0){$\ast$}}
\put(973,655){\makebox(0,0){$\ast$}}
\put(992,665){\makebox(0,0){$\ast$}}
\put(979,676){\makebox(0,0){$\ast$}}
\put(1037,675){\makebox(0,0){$\ast$}}
\put(1057,685){\makebox(0,0){$\ast$}}
\put(1031,686){\makebox(0,0){$\ast$}}
\put(1070,675){\makebox(0,0){$\ast$}}
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\multiput(1098.35,294.58)(-33.367,0.492){21}{\rule{25.933pt}{0.119pt}}
\multiput(1152.17,293.17)(-721.174,12.000){2}{\rule{12.967pt}{0.400pt}}
\multiput(294.00,235.58)(0.967,0.499){139}{\rule{0.872pt}{0.120pt}}
\multiput(294.00,234.17)(135.190,71.000){2}{\rule{0.436pt}{0.400pt}}
\multiput(1069.00,222.61)(1.355,0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(1069.00,221.17)(4.855,3.000){2}{\rule{0.517pt}{0.400pt}}
%\put(1063,215){\makebox(0,0){ 400}}
\multiput(1202.68,292.94)(-0.920,-0.468){5}{\rule{0.800pt}{0.113pt}}
\multiput(1204.34,293.17)(-5.340,-4.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(940.00,224.60)(0.774,0.468){5}{\rule{0.700pt}{0.113pt}}
\multiput(940.00,223.17)(4.547,4.000){2}{\rule{0.350pt}{0.400pt}}
\put(933,217){\makebox(0,0){ 420}}
\multiput(1073.68,294.94)(-0.920,-0.468){5}{\rule{0.800pt}{0.113pt}}
\multiput(1075.34,295.17)(-5.340,-4.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(810.00,226.60)(0.920,0.468){5}{\rule{0.800pt}{0.113pt}}
\multiput(810.00,225.17)(5.340,4.000){2}{\rule{0.400pt}{0.400pt}}
\put(804,219){\makebox(0,0){ 440}}
\multiput(944.09,296.94)(-0.774,-0.468){5}{\rule{0.700pt}{0.113pt}}
\multiput(945.55,297.17)(-4.547,-4.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(682.00,228.60)(0.920,0.468){5}{\rule{0.800pt}{0.113pt}}
\multiput(682.00,227.17)(5.340,4.000){2}{\rule{0.400pt}{0.400pt}}
\put(676,221){\makebox(0,0){ 460}}
\multiput(813.71,298.95)(-1.355,-0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(815.86,299.17)(-4.855,-3.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(553.00,230.60)(0.774,0.468){5}{\rule{0.700pt}{0.113pt}}
\multiput(553.00,229.17)(4.547,4.000){2}{\rule{0.350pt}{0.400pt}}
\put(546,223){\makebox(0,0){ 480}}
\multiput(685.71,300.95)(-1.355,-0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(687.86,301.17)(-4.855,-3.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(423.00,233.61)(1.355,0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(423.00,232.17)(4.855,3.000){2}{\rule{0.517pt}{0.400pt}}
\put(417,226){\makebox(0,0){ 500}}
\multiput(556.26,302.95)(-1.132,-0.447){3}{\rule{0.900pt}{0.108pt}}
\multiput(558.13,303.17)(-4.132,-3.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(294.00,235.61)(1.355,0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(294.00,234.17)(4.855,3.000){2}{\rule{0.517pt}{0.400pt}}
\put(288,228){\makebox(0,0){ 520}}
\multiput(426.71,304.95)(-1.355,-0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(428.86,305.17)(-4.855,-3.000){2}{\rule{0.517pt}{0.400pt}}
\put(1089,221){\makebox(0,0)[l]{ 270}}
\put(1049.0,222.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(294,233.67){\rule{4.818pt}{0.400pt}}
\multiput(294.00,234.17)(10.000,-1.000){2}{\rule{2.409pt}{0.400pt}}
\put(1069,231.67){\rule{4.818pt}{0.400pt}}
\multiput(1079.00,231.17)(-10.000,1.000){2}{\rule{2.409pt}{0.400pt}}
%\put(1108,232){\makebox(0,0)[l]{ 275}}
\put(314.0,245.0){\rule[-0.200pt]{4.577pt}{0.400pt}}
%\put(1128,242){\makebox(0,0)[l]{ 280}}
\put(1088.0,243.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(333.0,255.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(1147,252){\makebox(0,0)[l]{ 285}}
\put(1108.0,253.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(353.0,265.0){\rule[-0.200pt]{4.577pt}{0.400pt}}
%\put(1167,262){\makebox(0,0)[l]{ 290}}
\put(1128.0,263.0){\rule[-0.200pt]{4.577pt}{0.400pt}}
\put(372,274.67){\rule{4.818pt}{0.400pt}}
\multiput(372.00,275.17)(10.000,-1.000){2}{\rule{2.409pt}{0.400pt}}
\put(1147,272.67){\rule{4.818pt}{0.400pt}}
\multiput(1157.00,272.17)(-10.000,1.000){2}{\rule{2.409pt}{0.400pt}}
%\put(1187,273){\makebox(0,0)[l]{ 295}}
\put(392.0,286.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(1167,282.67){\rule{4.577pt}{0.400pt}}
\multiput(1176.50,282.17)(-9.500,1.000){2}{\rule{2.289pt}{0.400pt}}
%\put(1206,283){\makebox(0,0)[l]{ 300}}
\put(411.0,296.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(1226,293){\makebox(0,0)[l]{ 305}}
\put(1186.0,294.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(431.0,306.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\end{picture}

